Multi-scale and Cross-scale Contrastive Learning for Semantic Segmentation

This work considers supervised contrastive learning for semantic segmentation. We apply contrastive learning to enhance the discriminative power of the multi-scale features extracted by semantic segmentation networks. Our key methodological insight is to leverage samples from the feature spaces emanating from multiple stages of a model's encoder itself requiring neither data augmentation nor online memory banks to obtain a diverse set of samples. To allow for such an extension we introduce an efficient and effective sampling process, that enables applying contrastive losses over the encoder's features at multiple scales. Furthermore, by first mapping the encoder's multi-scale representations to a common feature space, we instantiate a novel form of supervised local-global constraint by introducing cross-scale contrastive learning linking high-resolution local features to low-resolution global features. Combined, our multi-scale and cross-scale contrastive losses boost performance of various models (DeepLabV3, HRNet, OCRNet, UPerNet) with both CNN and Transformer backbones, when evaluated on 4 diverse datasets from natural (Cityscapes, PascalContext, ADE20K) but also surgical (CaDIS) domains. Our code is available at https://github.com/RViMLab/MS_CS_ContrSeg. datasets from natural (Cityscapes, PascalContext, ADE20K) but also surgical (CaDIS) domains.

==> tab/pseudocode.tex <==
% \resizebox{0.8\linewidth}{!}{
\begin{algorithm*}[ht]
\SetAlgoLined
    \PyComment{Assume an encoder $f_{enc}$ and $f_{proj}$ being a set of $S$ projection heads each mapping to feature space of dimension $d$}\\
    \PyComment{$(X, \Tilde{Y})$ a batch of images and down-sampled labels} \\
    \PyComment{$S$ being the number of scales, $S_{pairs}$ being the scale ids for scale pairs} \\
    \PyComment{$b$ being the batch size}\\
    \PyComment{$h_{i},w_{i},c_i$ being the height, width and channels of each feature of $f_{enc}$}\\
    \quad\\
    \PyCode{$\ca{L} = 0$} \PyComment{init loss}\\
    \PyCode{A = [ ]} \PyComment{empty list to be populated with anchors/labels for cross-scale loss}\\ 
    \quad\\
    \PyComment{forward encoder} \\
    $F_{i=1,...,S} = f_{enc}(X)$  \PyComment{$b,h_{i},w_{i},c_i$} \\
    \PyComment{forward projection heads} \\
    $Z_{i=1,...,S} = f_{proj}(F_{i=1,...,S})$  \PyComment{$b,h_i,w_i,d$} \\
    \quad\\
    \PyComment{Computation of multi-scale loss} \\
    \PyCode{for i in range($S$):} \\
    \Indp   % start indent
        \PyComment{Sample Anchors} \\
        \PyComment{$N_i$ is the number of class instances in batch (with repetition) at scale i} \\ \PyComment{$K_i$ is the samples from the class with min samples in batch} \\
        \PyCode{$\ca{A}_i, Y_i$ = SampleAnchors($X, \Tilde{Y}$, i)} \PyComment{$N_i,K_i,d$ and $N_i$}  \\ 
        
        \PyComment{$Y_i$ are the label ids of the sampled anchors at scale i} \\
        \PyComment{Determine Positives and Negatives for each anchor in $\ca{A}_i$} \\
        
        \PyCode{$\ca{N}$, $\ca{P}$ = NegPos($Y_i$)}  \PyComment{$N_i, N_i$} and \PyComment{$N_i, N_i$} \\
        \PyComment{Compute loss of equation $1$ (main paper)} \\
        \PyCode{$\Lc_c(\ca{A}_i) =$ InfoNCE($\ca{A}_i$, $\ca{N}$, $\ca{P}$)}
        
        \PyComment{Overall multi-scale loss is weighted comb. of the loss at each scale} \\

        \PyCode{$\ca{L}$ += $\Lc_c(\ca{A}_i)$ * $w_i$} \\
        \PyCode{if i in scale pairs:} \PyCode{A.append(($\ca{A}_i$, $Y_i$))} \\

    \Indm % end indent
    \quad\\
    \PyComment{Computation of cross-scale loss} \\
    \PyCode{for p, (i,j) in enumerate($S_{pairs}$):} \\
    \Indp   % start indent
            \PyCode{($\ca{A}_i$, $Y_i$), ($\ca{A}_j$, $Y_j$) = A[i], A[j]} \\
            \PyComment{For each anchor in $\ca{A}_i$ determine Positives and Negatives from $\ca{A}_j$ }\\
            \PyCode{$\ca{N}$, $\ca{P}$ = NegPos($Y_i$,$Y_j$)}  \PyComment{$N_i, N_j$} and \PyComment{$N_i, N_j$} \\
            \PyCode{$\Lc_c(\ca{A}_i, \ca{A}_j$) = InfoNCE($\ca{A}_i$, $\ca{A}_j$, $\ca{N}$, $\ca{P}$)} \\
            \PyComment{Overall cross-scale loss is weighted comb. of the loss at each pair} \\
            \PyCode{$\ca{L}$ += $\Lc_c(\ca{A}_i, \ca{A}_j)$ * $w_p$} \\

    \Indm % end indent

\caption{Pseudo-code for computing our multi- and cross-scale losses.}
\label{algo:pseudo}
\end{algorithm*}
% }
